Magnetic twist profile inside magnetic clouds derived with a superposed epoch analysis

Magnetic clouds (MCs) are large-scale interplanetary transient structures in the heliosphere that travel from the Sun into the interplanetary medium. The internal magnetic field lines inside the MCs are twisted, forming a flux rope (FR). This magnetic field structuring is determined by its initial solar configuration, by the processes involved during its eruption from the Sun, and by the dynamical evolution during its interaction with the ambient solar wind. One of the most important properties of the magnetic structure inside MCs is the twist of the field lines forming the FR (the number of turns per unit length). The detailed internal distribution of twist is under debate mainly because the magnetic field (B) in MCs is observed only along the spacecraft trajectory, and thus it is necessary to complete observations with theoretical assumptions. Estimating the twist from the study of a single event is difficult because the field fluctuations significantly increase the noise of the observed B time series and thus the bias of the deduced twist. The superposed epoch applied to MCs has proven to be a powerful technique, permitting the extraction of their common features, and removing the peculiarity of individual cases. We apply a superposed epoch technique to analyse the magnetic components in the local FR frame of a significant sample of moderately asymmetric MCs observed at 1 au. From the superposed profile of B components in the FR frame, we determine the typical twist distribution in MCs. The twist is nearly uniform in the FR core (central half part), and it increases moderately, up to a factor two, towards the MC boundaries. This profile is close to the Lundquist field model limited to the FR core where the axial field component is above about one-third of its central value.

==> labels_superposed.tex <==
Useful to write the Fig., Eq. and Sect. labels with copy/paste.   
Of course to keep updated.
 
\sect{Introduction}

\sect{Data}
  \sect{Data_MC}
  \sect{Data_Examples}
  \sect{Data_CB}
     \eq{CB_definition}
     \eq{CB_definition_b}
  \sect{Data_MC_selection}
  \sect{Data_Comparison_L_MV}
  
\sect{SEA}
  \sect{SEA_method}
  \sect{SEA_profiles}
  \sect{SEA_around_MCs}
  \sect{SEA_Fitting}
  \sect{SEA_twist}

\sect{Conclusions}

\sect{FRframe} % Appendix A
     \eq{B_FR}
     \eq{rc}
     \eq{B_Lundquist}
     \eq{B_GH}

\sect{Table}. % Appendix B

Fig. 1 \fig{events}
Fig. 2 \fig{histogram_CB}
Fig. 3 \fig{histogram_p}
Fig. 4 \fig{comparison_orientation_L_vs_MV}
Fig. 5 \fig{superposed_L}
Fig. 6 \fig{superposed_L_vs_MV}
Fig. 7 \fig{fit_B_SEA}
Fig. 8 \fig{twist_vs_x}
Fig. 9 \fig{twist_vs_r}
Fig.A.1 \fig{coordinate_system}

Table 1    \tab{fit}
Table B.1  \tab{cases}

